Derivative-Agnostic Inference of Nonlinear Hybrid Systems

This paper addresses the problem of inferring a hybrid automaton from a set of input-output traces of a hybrid system exhibiting discrete mode switching between continuously evolving dynamics. Existing approaches mainly adopt a derivative-based method where (i) the occurrence of mode switching is determined by a drastic variation in derivatives and (ii) the clustering of trace segments relies on signal similarity -- both subject to user-supplied thresholds. We present a derivative-agnostic approach, named Dainarx, to infer nonlinear hybrid systems where the dynamics are captured by nonlinear autoregressive exogenous (NARX) models. Dainarx employs NARX models as a unified, threshold-free representation through the detection of mode switching and trace-segment clustering. We show that Dainarx suffices to learn models that closely approximate a general class of hybrid systems featuring high-order nonlinear dynamics with exogenous inputs, nonlinear guard conditions, and linear resets. Experimental results on a collection of benchmarks indicate that our approach can effectively and efficiently infer nontrivial hybrid automata with high-order dynamics yielding significantly more accurate approximations than state-of-the-art techniques.

==> def.tex <==
% !TEX root = main.tex

\RequirePackage{todonotes}

%%Notes
\newcommand{\cmscomment}[1]{\todo[color=blue!10,size=\small,fancyline,author=CMS]{#1}\xspace}
\newcommand{\cmscommentinline}[1]{\todo[inline,color=blue!10,author=CMS]{#1}\xspace}
\newcommand{\atcms}{\colorbox{blue!10}{\textbf{@CMS}}}

\newcommand{\yhzcomment}[1]{\todo[color=blue!25,size=\small,fancyline,author=YHZ]{#1}\xspace}
\newcommand{\yhzcommentinline}[1]{\todo[inline,color=blue!25,author=YHZ]{#1}\xspace}
\newcommand{\atyhz}{\colorbox{blue!25}{\textbf{@YHZ}}}

\newcommand{\mbhcomment}[1]{\todo[color=orange!25,size=\small,fancyline,author=MBH]{#1}\xspace}
\newcommand{\mbhcommentinline}[1]{\todo[inline,color=orange!25,author=MBH]{#1}\xspace}
\newcommand{\atmbh}{\colorbox{orange!25}{\textbf{@MBH}}}

\newcommand{\ajcomment}[1]{\todo[color=yellow!25,size=\small,fancyline,author=AJ]{#1}\xspace}
\newcommand{\ajcommentinline}[1]{\todo[inline,color=yellow!25,author=AJ]{#1}\xspace}
\newcommand{\ataj}{\colorbox{yellow!25}{\textbf{@AJ}}}

\newcommand{\znjcomment}[1]{\todo[color=yellow!25,size=\small,fancyline,author=ZNJ]{#1}\xspace}
\newcommand{\znjcommentinline}[1]{\todo[inline,color=yellow!25,author=ZNJ]{#1}\xspace}
\newcommand{\atznj}{\colorbox{yellow!25}{\textbf{@ZNJ}}}

% Colored marks
\newcommand{\Cmark}{\textcolor{ForestGreen}{\ding{51}}}%
\newcommand{\Xmark}{\textcolor{Maroon}{\ding{55}}}%
\newcommand{\NAmark}{\textcolor{Maroon}{\textbf{?}}}%

% Uncolored marks
\newcommand{\CmarkB}{\ding{51}}%
\newcommand{\XmarkB}{\ding{55}}%
\newcommand{\NAmarkB}{\textbf{?}}%

% Extra colors
\definecolor{customgreen}{HTML}{00731e}  % green
\definecolor{customorange}{HTML}{ff962e} % orange
\definecolor{custompink}{HTML}{e96db6}   % pink
\definecolor{customcyan}{HTML}{00b8c6} % cyan

\newcommand{\ourmethod}{\textnormal{\textsc{Dainarx}}\xspace}
\newcommand{\benchmark}[1]{\textnormal{\texttt{#1}}}
\newcommand{\hdt}{\ensuremath{\textit{HDT}_{c}}\xspace}
\newcommand{\diffmax}{\ensuremath{\textit{Diff}_{\textit{max}}}\xspace}
\newcommand{\diffavg}{\ensuremath{\textit{Diff}_{\textit{avg}}}\xspace}

% Reals, Rationals...
\newcommand{\Nats}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\NatsInf}{\mathbb{N}^\infty\xspace}
\newcommand{\PosNats}{\ensuremath{\mathbb{N}_{>0}}\xspace}
\newcommand{\Ints}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\Rats}{\ensuremath{\mathbb{Q}}\xspace}
\newcommand{\Reals}{\mathbb{R}}
\newcommand{\StrictPosReals}{\mathbb{R}_{>0}}
\newcommand{\PosReals}{\mathbb{R}_{> 0}}
\newcommand{\PosRats}{\mathbb{Q}_{\geq 0}}
\newcommand{\PosRealsInf}{\mathbb{R}_{> 0}^\infty}

\newcommand{\RR}{\Reals}
\newcommand{\NN}{\Nats}
\newcommand{\bigO}{\ensuremath{\mathcal{O}}\xspace}

\newcommand{\mybar}[3]{%
    \mathrlap{\hspace{#2}\overline{\scalebox{#1}[.9]{\phantom{\ensuremath{#3}}}}}\ensuremath{#3}
}

%% hybrid systems
\renewcommand{\ha}{\ensuremath{\mathcal{H}}\xspace}
\newcommand{\haLearned}{\ensuremath{\mybar{0.6}{3pt}{\mathcal{H}}}\xspace}
%\newcommand{\haLearned}{\ensuremath{\bar{\mathcal{H}}}\xspace}
\newcommand{\modes}{\ensuremath{Q}\xspace}
\newcommand{\vars}{\ensuremath{V}\xspace}
\newcommand{\varsO}{\ensuremath{X}\xspace}
\newcommand{\varsI}{\ensuremath{U}\xspace}
\newcommand{\flows}{\ensuremath{\mathcal{F}}\xspace}
\newcommand{\inv}{\ensuremath{\mathit{Inv}}\xspace}
\newcommand{\init}{\ensuremath{\mathit{Init}}\xspace}
\newcommand{\trans}{\ensuremath{\mathcal{T}}\xspace}

% \newcommand{\domain}{\mathcal{D}}
% \newcommand{\init}{\mathcal{X}_0}
% \newcommand{\initBound}{\mathcal{I}}
% \newcommand{\unsafe}{\mathcal{X}_u}
% \newcommand{\unsafek}{\mathcal{X}_{u,k}}
% \newcommand{\unsafeBound}{\mathcal{U}}
% \newcommand{\reach}{\mathcal{R}}
% \newcommand{\compactSet}{\mathcal{C}}
% \newcommand{\invt}{\Psi}
% \newcommand{\ball}{\mathfrak{B}}
% %\newcommand{\tbound}{\mathcal{T}}
% \newcommand{\tbound}{T}

\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}

\newcommand{\data}{\ensuremath{\mathcal{D}}\xspace}
\newcommand{\cpoints}{\ensuremath{\textit{CP}}\xspace}
\newcommand{\lastcp}{\ensuremath{\textit{last\_cp}}\xspace}
\newcommand{\midElement}{\ensuremath{\textit{mid}}\xspace}
\newcommand{\lb}{\ensuremath{\textit{lb}}\xspace}
\newcommand{\rb}{\ensuremath{\textit{rb}}\xspace}
\newcommand{\segments}{\ensuremath{\textit{Seg}}\xspace}
\newcommand{\segment}{\ensuremath{\textit{seg}}\xspace}
% \newcommand{\clusters}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\windowSize}{\ensuremath{w}\xspace}

\newcommand{\samples}{\ensuremath{Z}\xspace}
\newcommand{\samplesPos}{\ensuremath{Z^+}\xspace}
\newcommand{\samplesNeg}{\ensuremath{Z^-}\xspace}
\newcommand{\targetMode}{\ensuremath{\mathcal{M}}\xspace}

\newcommand{\narx}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\narxIns}{\ensuremath{N}\xspace}
\newcommand{\narxInsSet}{\ensuremath{\langle \narx \rangle}\xspace}
\newcommand{\cmat}{\ensuremath{\mathcal{A}}\xspace}
\newcommand{\cmatIns}{\ensuremath{\Lambda}\xspace}

\newcommand{\Omatrix}{\ensuremath{O}\xspace}
\newcommand{\Dmatrix}{\ensuremath{D}\xspace}

\newcommand{\proj}[2]{\ensuremath{#1\vert_{#2}}\xspace}
\newcommand{\projO}[1]{\proj{#1}{\varsO}}
\newcommand{\projI}[1]{\proj{#1}{\varsI}}

\newcommand{\traceCTH}{\ensuremath{\rho}\xspace}
\newcommand{\traceDT}{\ensuremath{\xi}\xspace}
\newcommand{\traceDTLen}{\ensuremath{\ell}\xspace}
\newcommand{\traceNARX}{\ensuremath{\zeta}\xspace}
\newcommand{\signal}{\ensuremath{\sigma}\xspace}

\newcommand{\xx}{\mathbf{x}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\zz}{\mathbf{z}}
\newcommand{\aaa}{\mathbf{a}}
\newcommand{\sss}{\mathbf{s}}
\newcommand{\va}{\mathbf{\alpha}}
\newcommand{\sol}{{\bm \zeta}}
%\newcommand{\vsol}{{\bm \zeta}}
%\newcommand{\xx}{\bm{x}}
\newcommand{\uu}{\mathbf{u}}
\newcommand{\rr}{\mathbf{r}}
\renewcommand{\vv}{\mathbf{v}}
\newcommand{\ttt}{\mathbf{t}}
\newcommand{\dd}{\mathbf{d}}
%\newcommand{\zz}{\mathbf{0}}
\newcommand{\one}{\mathbf{1}}
\newcommand{\zmatrix}{O}
%\newcommand{\zmatrix}{\mathit{0}}

\newcommand{\psd}{PSD}

\newcommand{\ff}{{\bm f}}
\newcommand{\ffk}[1]{{\bm f}_{\!#1}}
%\newcommand{\ff}{\mathbf{f}}
%\newcommand{\fg}{\mathbf{g}}
\newcommand{\fg}{{\bm g}}
\newcommand{\pphi}{{\bm \phi}}
%\newcommand{\pphi}{\mathbf{\phi}}

\newcommand{\XX}{\mathrm{X}}
\newcommand{\YY}{\mathrm{Y}}

\newcommand{\quadraticVar}{Z}

\newcommand{\toolname}[1]{\textsf{#1}}
\newcommand{\expname}[1]{\textnormal{\textsf{#1}}}

\newcommand{\LieBound}{N_{B\mkern-1mu, \mkern-.2mu\ff}}
\newcommand{\LieBoundBi}{N_{B_k\mkern-1mu, \mkern-.2mu\ff_{\mkern-2mu k}}}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}
\DeclarePairedDelimiter\normsqrt{\lVert}{\rVert}
\DeclarePairedDelimiter\norm{\lVert}{\rVert_2}
\newcommand{\normDisplaysqrt}[1]{\left\lVert#1\right\rVert}
\newcommand{\normDisplay}[1]{\left\lVert~#1~\right\rVert_2}
\newcommand{\normOneDisplay}[1]{\left\lVert~#1~\right\rVert_1}
\newcommand{\normDTWDisplay}[1]{\left\lVert~#1~\right\rVert_{\text{DTW}}}

\newcommand{\hadamard}{\ensuremath{\circ}\xspace}

%\newcommand{\norm}[1]{\left\lvert#1\right\rvert}
\newcommand{\normbrace}[1]{\bigg\lVert#1\bigg\rVert}
\newcommand{\normshorter}[1]{\big\lvert#1\big\rvert}
\newcommand{\infnorm}[1]{\left\lvert#1\right\rvert_\infty}
\newcommand{\infnormbrace}[1]{\bigg\lvert#1\bigg\rvert_\infty}
\newcommand{\infnormshorter}[1]{\big\lvert#1\big\rvert_\infty}
%\newcommand{\abs}[1]{\left\lvert#1\right\rvert}
\newcommand*\from{\colon}
\DeclareMathOperator{\dif}{\,d\!}
\newcommand*{\transpose}{\mathsf{T}}
\newcommand*{\diag}{\mathit{diag}}
\newcommand{\TAG}[1]{{\tag*{[\small{{#1}}]}}}

%spaced relations
\newcommand{\ppreceq}{~{}\preceq{}~}
\newcommand{\ssucceq}{~{}\succeq{}~}
\newcommand{\defeq}{{}\triangleq{}}
\newcommand{\ddefeq}{\ {}\defeq{}\ }
\newcommand{\eeq}{~{}={}~}
\renewcommand{\mmapsto}{~{}\mapsto{}~}
\newcommand{\eequiv}{~{}\equiv{}~}
\newcommand{\pplus}{~{}+{}~}
\newcommand{\ccdot}{~{}\cdot{}~}
\newcommand{\llongrightarrow}{~{}\longrightarrow{}~}
\newcommand{\qlongrightarrow}{\quad{}\longrightarrow{}\quad}
\newcommand{\qqlongrightarrow}{\qquad{}\longrightarrow{}\qquad}
\newcommand{\mmid}{~{}\mid{}~}
\newcommand{\qmid}{\quad{}|{}\quad}
\newcommand{\tto}{~{}\to{}~}
\newcommand{\uuplus}{\,{}\uplus{}\,}
\newcommand{\nneq}{~{}\neq{}~}
\newcommand{\qeq}{\quad{}={}\quad}
\newcommand{\qqeq}{\qquad{}={}\qquad}
\newcommand{\lleq}{~{}\leq{}~}
\newcommand{\LL}{~{}<{}~}
\newcommand{\GG}{~{}>{}~}
\newcommand{\ggeq}{~{}\geq{}~}
\newcommand{\aand}{\ \ \textnormal{and}\ \ }
\newcommand{\qand}{\ \quad\textnormal{and}\quad\ }
\newcommand{\ssqsubseteq}{~{}\sqsubseteq{}~}
\newcommand{\iimplies}{~{}\implies{}~}
\newcommand{\mmodels}{~{}\models{}~}
\newcommand{\nnotmodels}{~{}\not\models{}~}
\newcommand{\iin}{~{}\in{}~}
\newcommand{\nnotin}{~{}\not\in{}~}
\newcommand{\wwedge}{~{}\wedge{}~}
\newcommand{\vvee}{~{}\vee{}~}

\newcommand{\minimize}{\mathtt{minimize}}
\newcommand{\subj}{\mathtt{subject~to}}
\newcommand{\qfor}{\quad\text{for}~}
\newcommand{\innerp}{\vcenter{\hbox{\scriptsize$\bullet$}}}
% \newcommand{\trace}{\mathit{tr}}

\newcommand{\closure}[2][3]{{}\mkern#1mu\overline{\mkern-#1mu#2}}
\newcommand{\boundary}{\partial}
\newcommand{\interior}{\mathsf{o}}

% rewriting \Re and \Im from amsmath
\renewcommand{\Re}{\mathfrak{R}}
\renewcommand{\Im}{\mathfrak{I}}
\newcommand{\iu}{{\mathrm{i}\mkern1mu}}
\renewcommand{\exp}[1]{\mathrm{e}^{#1}}

\newcommand{\basin}{\mathfrak{B}}

\newcommand{\lap}[1]{\mathcal{L}\{#1\}}
\newcommand{\bigo}[1]{\mathcal{O}\left(#1\right)}

%non-italic enumerate numbers in definitions
%\AtBeginEnvironment{definition}{\setlist[enumerate, 1]{font=\upshape}}

%% amsthm configurations


%redefine QED mark, make it smaller
\def\boxforqed{\hbox{{\small $\square$}}}
\def\qed{\ifmmode\else\unskip\quad\fi\boxforqed}
\def\smartqed{\def\qed{\ifmmode\boxforqed\else{\unskip\nobreak\hfil
			\penalty50\hskip1em\null\nobreak\hfil\boxforqed
			\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}}

\smartqed  % flush right qed marks, e.g. at end of proof

%%introduce end mark for theorem-like environments
%\def\triangleforqed{\hbox{$\lhd$}}
%\def\qedT{\ifmmode\else\unskip\quad\fi\triangleforqed}
%\def\smartqedT{\def\qedT{\ifmmode\triangleforqed\else{\unskip\nobreak\hfil
%			\penalty50\hskip1em\null\nobreak\hfil\triangleforqed
%			\parfillskip=0pt\finalhyphendemerits=0\endgraf}\fi}}
%
%\smartqedT  % flush right qedT marks, e.g. at end of theorem-environments

%for qed mark compatible within displaymath
\def\boxforqed{\hbox{{\small $\square$}}}
\makeatletter
\DeclareRobustCommand{\qedBB}{%
	\ifmmode
	\eqno \def\@badmath{$$}%$$
	\let\eqno\relax \let\leqno\relax \let\veqno\relax
	\hbox{\boxforqed}%
	\else
	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
	\quad\hbox{\boxforqed}%
	\fi
}
\makeatother

%for qedT mark compatible within displaymath
% \def\triangleforqed{\hbox{$\blacktriangleleft$}}
\def\triangleforqed{\hbox{$\lhd$}}
 \makeatletter
 \DeclareRobustCommand{\qedT}{%
 	\ifmmode
 	\eqno \def\@badmath{$$}%$$
 	\let\eqno\relax \let\leqno\relax \let\veqno\relax
 	\hbox{\triangleforqed}%
 	\else
 	\leavevmode\unskip\penalty9999 \hbox{}\nobreak\hfill
 	\quad\hbox{\triangleforqed}%
 	\fi
 }
 \makeatother

%for equation labels with tags
\makeatletter
\newcommand{\owntag}[2][\relax]{% \owntag[short label]{tag}
	\ifx#1\relax\relax\def\owntag@name{#2}\else\def\owntag@name{#1}\fi% base label
	\refstepcounter{equation}\tag{\theequation, \small{#2}}%
	\expandafter\ltx@label\expandafter{eqn:\owntag@name}%
	\edef\@currentlabel{\theequation, #2}\expandafter\ltx@label\expandafter{Eq:\owntag@name}%
	\def\@currentlabel{#2}\expandafter\ltx@label\expandafter{tag:\owntag@name}%
}
\makeatother

